MapComp: A Secure View-based Collaborative Analytics Framework for Join-Group-Aggregation

Join-group-aggregation (JGA) queries are fundamental to data analytics, yet executing them collaboratively across different parties poses significant privacy risks. Secure multi-party computation (MPC) offers a cryptographic solution. However, existing MPC-based JGA approaches consider only a one-time query paradigm and suffer from significant performance bottlenecks. It executes expensive join operations from scratch across multiple queries and employs inefficient group-aggregation (GA) protocols, both of which hinder their practical use for scalable, real-time analysis. This paper introduces MapComp, a novel view-based framework to facilitate JGA queries for secure collaborative analytics. Through specially crafted materialized views for join and novel design of GA protocols, MapComp removes duplicate join workload and expedites subsequent GA, improving the efficiency of JGA query execution. To address the challenge of continuous data updates, our materialized view offers payload-independence feature and provides significant efficiency improvements in view refreshing with free MPC overhead. This feature, on the other hand, also allows further acceleration for GA, where we devise multiple novel protocols that outperform prior works. Notably, our work represents the first endeavor to expedite secure collaborative JGA queries using materialized views. Our rigorous experiments demonstrate a significant advantage of MapComp, achieving up to a 308.9x improvement in efficiency over the baseline in real-world query simulations. Moreover, our optimized GA protocols achieve up to a 1140.5x improvement compared to prior oblivious sorting-based solutions.

==> abstract.tex <==



Numerous businesses can gain benefits from collaborative analysis of databases owned by diverse entities, yet privacy concerns pose the primary obstacle. A promising solution is to perform secure queries with secure multi-party computation (MPC). However, existing MPC-based approaches generally adopt the paradigm of one-time query processing with a heavy workload, which incurs a significant overhead and limits its practical application.

% one-time

% When dealing with multiple similar queries with dynamically updated databases, such existing schemes incur significant performance overheads as they require repeated executions over a whole database. 

% Private data federation enables mutually distrustful parties to query over collective data while preserving data privacy. 

% 原版：The blueprint of a private data federation enables multiple parties to work together to provide query-answering on the union of their data, where privacy concerns have become a major stymie. A promising solution is to perform secure queries leveraging secure multi-party computation (MPC) techniques. Unfortunately,  when dealing with dynamically updating databases and queries, MPC-based approaches incur a significant performance overhead as they require repeated executions over the whole database to preserve access patterns. \LWR{See comments in the source code.}

% 第一小段：Private data federation enables mutually distrustful parties to query over the collective data while preserving data privacy and secrecy. A promising solution is to perform secure queries with secure multi-party computation (MPC) techniques. However, MPC generally considers the one-time query processing paradigm. When dealing with dynamically updating databases and queries, such paradigm incurs a significant performance overhead as they require repeated executions over the whole database. 
% 逻辑：private data federation能保护隐私也能查询。一般private data federation都是基于MPC构造的。MPC一般考虑单次问询。当数据和问询持续变化时，当前解决方案需要在整个数据库上执行问询，开销较大。

This paper introduces MapComp, a novel view-based framework to facilitate secure join-group-aggregation (JGA) queries. The JGA pattern captures numerous real-world statistical queries, making optimization crucial for secure collaborative analytics. MapComp leverages a specially crafted structure generated by \textit{mapping} as a materialized view to allow re-use or pre-computation of join process. This mapping feature also offers \textit{payload independence}, enabling free record updating and further optimizations for subsequent \textit{group aggregation}. To instantiate MapComp, we realize \textit{mapping} with a tunable three-way trade-off between information leakage and efficiency using private set operation protocols (\eg Private-ID), and devise multiple novel protocols for \textit{group-aggregation} that outperform existing methods by leveraging ideas of sorting optimizations and bitmaps. Notably, our work represents the first endeavor to expedite secure collaborative JGA queries using materialized views that support efficient record updating. Our experiments demonstrate MapComp's significant advantage, achieving up to a $474\times$ improvement in speed compared to baseline when executing queries with the same join condition six times. Additionally, the optimized group-aggregation protocols yield up to $208\times$ efficiency improvement over the baseline workload.


% Our experiments confirm MapComp's advantage, which is up to $474\times$ faster than the baseline after executing queries with the same join table 6 times. Moreover, the optimized group-by aggregation protocols provide up to xxx efficiency improvement over baseline.

% offers up to xxx performance advantage over baseline 

% In this paper, we focus on facilitating secure Join-Group-Aggregate (JGA) queries, which cover the most commonly used statistical queries in private data federation. To this end, we propose MapComp, a novel framework that 

% 原版：In this work, we propose MapComp, a novel framework for secure join-group-aggregate queries that support efficient answering for dynamic updating of data and queries. We proposed a lightweight materialized view that allows the parties to cache important intermediate outputs, thus subsequent queries with updated database or query conditions can be accelerated with leaner processing.  We divided join-group-aggregate into two main processes: \textit{mapping} and \textit{group-aggregate}. \textit{Mapping} provides a lightweight materialized to minimize the overhead of subsequent workload, and we provide a tunable three-way trade-off between information leakage and efficiency. To support group-by aggregation, \textit{group-aggregate} builds multiple efficient protocols based on mapping to cover different cases of data inputs \LWR{This is not clear, what is the meaning of different data inputs?}. To the best of our knowledge, our work is the first to support efficient answering in case of modification or deletion of data, as well as query condition updating without re-running the whole protocol. Our experiments show that \hfnote{xxx}. 

% 这段写的还可以，有几个地方逻辑不太通：（1）第一句话，为什么我们关注join-group-aggregate？需要补半句话：which covers most commonly used queries in private data federtaion.（2）We divided join-group-aggregate into two main processes。后面跟的两句话要对仗，即：\textit{Mapping} provides a ..., \textit{Group-aggregate} provides了什么。

==> mapping_dumped.tex <==

% In this section, we describe what is mapping and how to securely generate it.
In this section, we first define mapping and discuss the security levels of mapping protocols. Then we present the constructions of mapping achieving different security levels.
We first consider the mapping for the PK-PK join and leave the discussion of supporting PK-FK join in \S \ref{sec:pk-fk} since it is closely related to the design group aggregation protocol.

% \subsection{Security levels and simple constructions of mapping}
\subsection{Definition and Security Levels of Mapping}
\label{sec:revisit}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/mappingExampleNew.pdf}
    \vspace{-0.1in}
    \caption{An example of mapping, where $E = (1, 0, 0, 1)$.}
    \vspace{-0.35in}
    \label{fig:mapExample}
\end{figure}

% Given two sets $X$ and $Y$ owned by two parties $\alice$ and $\bob$ respectively, a mapping protocol outputs $\shareb{E}_0$ and $\pi_a$ to $\alice$, $\shareb{E}_1$ and $\pi_b$ to $\bob$, where $\pi_a, \pi_b$ are two injective functions, and $E$ is the intersection flag vector, and,
% \begin{enumerate}
%     \item $n_e = |E| = |\pi_b| = |\pi_a| \geq n_{xy}$.
%     \item $\pi_a : [n_e]\rightarrow [\mathsf{max}(n_e, n_x)]$, and $\forall x_i\in X\bigcap Y, i\in \pi_a$.
%     \item $\pi_b : [n_e]\rightarrow [\mathsf{max}(n_e, n_y)]$, and $\forall y_j\in X\bigcap Y, j\in \pi_b$.
%     \item The number of 1 in $E$ is $|X \bigcap Y|$; $x_{\pi_a(i)} = y_{\pi_b(i)}$ iff $e_i = 1$.
% \end{enumerate}
% For each pair $(x, y)$ with $x\in X, y\in Y$ and $x=y$, applying $\pi_a, \pi_b$ on $X, Y$ respectively will map $x, y$ into the same position $i$ with $e_i = 1$. 

% With such mapping protocols, $\alice$ and $\bob$ can use $X = \tablesym{R^0}[k]$ and $Y = \tablesym{R^1}[k]$ as the input, and permute self-owned databases with received $\pi_a, \pi_b$ respectively. Then, $\tablesym{J^0} = \pi_a\cdot \tablesym{R^0}$ and $\tablesym{J^1} = \pi_b \cdot \tablesym{R^1}$ are aligned based on join key $k$, such that the purpose of equal-join is achieved by horizontally concatenate $\tablesym{J^0}, \tablesym{J^1}$, where $\shareb{e_i}$ represents whether the $i^{th}$ tuple is valid (whether $\tablesym{J^0}[k] = \tablesym{J^1}[k]$).
% Since the join operation utilizing the result of mapping protocols does not involve the associated payload values during secure computation, the obtained result $\pi_a, \pi_b, \shareb{E}$ can be \textit{reusable} in multiple queries with the same equal-join condition. 

% The result of mapping protocols can be directly used to perform secure PK-PK join, such that the join operation involving two databases held by two parties respectively can be locally computed.
% Taking a joint query involving the join operation with the condition of $\tablesym{A}.x = \tablesym{B}.y$ and the computation on other attributes $\tablesym{A}.\tilde{x}, \tablesym{B}.\tilde{y}$ as an example, $\alice$ and $\bob$ can permute self-owned databases $\tablesym{A}$ and $\tablesym{B}$ with $\pi_a, \pi_b$ respectively. Then, $\tablesym{A'} = \pi_a\cdot \tablesym{A}$ and $\tablesym{B'} = \pi_b \cdot \tablesym{B}$ are aligned based on $x = y$, such that the purpose of equal-join is achieved and $\shareb{e_i}$ represents whether the value of join key attribute of $i_{th}$ rows of $\tablesym{A'}, \tablesym{B'}$ are the same.
% Since the join operation utilizing the result of mapping protocols does not involve the associated payload values during secure computation, the obtained result $\pi_a, \pi_b, \shareb{E}$ can be \textit{reusable} in multiple queries with the same equal-join condition. 

% Given the affinity of such protocols for secure join, the next question is how to build a mapping protocol and how to measure the magnitude of private information leaked by different constructions.

Given two sets $X$ and $Y$ owned by two parties $\alice$ and $\bob$ respectively, a mapping protocol outputs $(\shareb{E}_0, \pi_a)$ to $\alice$ and $(\shareb{E}_1, \pi_b)$ to $\bob$, where $\pi_a, \pi_b$ are two injective functions, $E$ is the intersection flag vector, and they satisfy:
\begin{enumerate}
    \item $n_e = |E| = |\pi_b| = |\pi_a| \geq |X\cap Y|$. 
    \item $\pi_a : [n_e]\rightarrow [\mathsf{max}(n_e, n_x)]$, and $\forall x_i\in X\cap Y, i\in \pi_a$.
    \item $\pi_b : [n_e]\rightarrow [\mathsf{max}(n_e, n_y)]$, and $\forall y_j\in X\cap Y, j\in \pi_b$.
    % \item The number of 1 in $E$ is $|X \bigcap Y|$. 
    \item $|\{e | e\in E, e = 1\}| = |X \cap Y|$;
    $x_{\pi_a(i)} = y_{\pi_b(i)}$ iff $e_i = 1$.
\end{enumerate}

The idea behind is straightforward. For each pair $(x, y)$ in the $X \cap Y$ (e.g. $x\in X, y\in Y$ and $x=y$), applying $\pi_a, \pi_b$ on $X, Y$ respectively will map $x, y$ into the same position $i$ with $e_i = 1$. Therefore, the common records are aligned and the PK-PK join is essentially achieved.  An example of mapping is shown in Fig.\ref{fig:mapExample}

% 原版：For each pair $(x, y)$ in the $X \cap Y$ (e.g. $x\in X, y\in Y$ and $x=y$), applying $\pi_a, \pi_b$ on $X, Y$ respectively will map $x, y$ into the same position $i$ with $e_i = 1$. It realizes mapping and  realizes the PK-PK join as mentioned in \S \ref{sec:mapOverview}. An example of mapping is shown in Fig.\ref{fig:mapExample}
% We refer to the protocols whose outputs satisfy the above property as mapping protocols. A protocol is defined to be fully secure if $E$ is not revealed to both parties and $n_e$ only depends on the input size, and each party's injective function $\pi_a$ (or $\pi_a$) is private to the other party. Thus, the fully secure mapping won't reveal any information about the other party's input.
    
We define three different security levels based on the revealed information of $E$. 

% 原版：In each security level, nothing else is leaked to parties besides those that can be simulated based on the revealed information specified below and the received injective function ($\pi_a$ or $\pi_b$).

\begin{itemize}
    \item \textbf{level-0}: $E$ is revealed to two parties, which means parties know the intersection of two input sets.
    \item \textbf{level-1}:  $E$ is secret to two parties, and $|E| = f(X, Y)$, where $f$ is a public deterministic function. The size of $E$ may leak some information about the input of the other party beyond the input size, \eg the intersection size or the union size.  
    \item \textbf{level-2}: $E$ is secret to two parties, and $|E| = f(n_x,n_y)$, where $f$ is a public deterministic function. We also say level-2 security is fully secure because the size of $E$ leaks nothing beyond the input sizes $n_x$ and $n_y$, which is assumed to be public.
    % 原版\item \textbf{level-2}: $E$ is secret to two parties, and $|E| = f(n_x,n_y)$, where $f$ is a public deterministic function.
\end{itemize}

% 原版：The protocol of the higher level has a smaller magnitude of privacy leakage.
% Since $|E|$ only depends on the input size and the received injective function ($\pi_a$ or $\pi_b$) is random to the other party, we also say the protocol of level-2 is fully secure.

% 原版：level-1}: $|E|$ depends on the inputs $X$ and $Y$, and $E$ is secret to both parties. It means $\alice$ or $\bob$ can learn some information about the input of the other party, such as the upper bound of intersection size, while the intersection is secret to both parties. 

\begin{figure}\small
    \framebox{\begin{minipage}{0.97\linewidth}
        \begin{trivlist}
            \item \textbf{Parameters:} $\alice$ with set $X$ and a length-$n_x$ permutation $\pi_a$, $\bob$ with set $Y$, where $|X| = n_x, |Y| = n_y$ and $n_x \geq n_y$ are public.
            
            \item \textbf{Functionality:} 
            Upon receiving $X, \pi_a$ from $\alice$ and $Y$ from $\bob$.
            \begin{enumerate}
                \item Uniformly samples a random length-$n_x$ permutation $\pi_b$, which satisfy that $\forall i\in[n_x]$, 
                
                    $\left\{
                        \begin{aligned}
                        \pi_b(i) \leq n_y \text{ and } y_{\pi_b(i)} = x_{\pi_a(i)} , ~& \text{if } x_{\pi_a(i)}\in X\cap Y &\\
                        \pi_b(i) > n_y \text{ or } y_{\pi_b(i)} \notin X\cap Y, ~& \text{if } x_{\pi_a(i)}\notin X\cap Y &
                        \end{aligned}
                        \right.$
            
                \item Uniformly samples $E^0, E^1 \in \{0, 1\}^{n_x}$, such that $\forall i\in[n_x]$, $e^0_i\oplus e^1_i = 1$ if $x_{\pi_a(i)}\in X\cap Y$, otherwise $e^0_i\oplus e^1_i = 0$.
                
                \item The functionality sends $E^0$ to $\alice$ and $E^1, \pi_b$ to $\bob$.
            \end{enumerate}
        \end{trivlist}
    \end{minipage}}
    \vspace{-0.1in}
    \caption{Ideal functionality of fully secure mapping $\functionsym{map}$.}
    \vspace{-0.15in}
    \label{function:mapping}	
\end{figure}

\begin{figure}\small
    \framebox{\begin{minipage}{0.97\linewidth}
        \begin{trivlist}

            \item \textbf{Parameters:} Party $\alice$ with set $X$ and a length-$n_x$ permutation $\pi_a$, party $\bob$ with set $Y$, where $|X| = n_x, |Y| = n_y$ and $n_x \geq n_y$.

            \item \textbf{Protocol:} 
            \begin{enumerate}
                \item Invoke $\functionsym{cpsi}$. $\alice$ acts as receiver with input $X$ and $\bob$ acts as sender with input $(Y, O)$, where $O=(1, 2, \dots, n_y)$. As the result, the parties get $\shareb{E'}, \share{Z'}$.
                
                \item Invoke $\functionsym{osn}^s$, where $\alice$ acts as receiver with input $\pi_a$. $(\shareb{E}, \share{Z})\leftarrow\functionsym{osn}^s(\pi_a, (\shareb{E'}, \share{Z'}))$.
                
                \item Invoke $\functionsym{cpsi}$, where $\alice$ acts as sender with input $(X, \emptyset)$ and $\bob$ acts as receiver with input $Y$. the parties get $\shareb{F'}$.

                \item If $n_x > n_y$, the parties extend $\share{F'}$ into a length-$n_x$ shared vector by padding shared zeros at the end of it.

                \item Invoke $\functionsym{shuffle}$. $(\shareb{F}, \share{L}) \leftarrow \functionsym{shuffle}(\shareb{F'}, \share{O'})$ where $O' = (1, 2, \dots, n_x)$.

                \item Compute $\share{\sigma_1}\leftarrow\functionsym{perGen}(\shareb{F'})$, $\share{P^1} \leftarrow \functionsym{invp}^\mathsf{s}(\share{\sigma_1}, \share{L})$.
                
                \item Compute $\share{\sigma_0}\leftarrow\functionsym{perGen}(\shareb{E})$,  $\share{P^0}\leftarrow\functionsym{perm}^\mathsf{s}(\share{\sigma_0}, \share{P^1})$.
                \item Compute a shared permutation $\share{\pi_b}$ with $\share{\pi_b(i)} = \functionsym{mux}(\shareb{e_i}, \share{z'_i}, \share{p^0_i})$ for $i\in[n_x]$, and reveal $\pi_b$ to $\bob$.
            \end{enumerate}
            \item \textbf{Output:} $\alice$ returns $\shareb{E}_0$ and $\bob$ returns $\pi_b, \shareb{E}_1$.
        \end{trivlist}
    \end{minipage}}
    \vspace{-0.05in}
    \caption{Fully secure mapping protocol $\protocolsym{map2}$.}
    \vspace{-0.15in}
    \label{protocol:mapping}	
\end{figure}

\begin{figure*}[t!]
\centering
\includegraphics[width=0.7\linewidth]{figs/mapping.pdf}
\vspace{-0.15in}
\caption{Example of $\protocolsym{map2}$ where the inputs are $X = (a, b, c, d), \pi_a = (3,2,4,1), Y = (c, a, f), n_x = 4, n_y = 3$.}
\vspace{-0.2in}
\label{fig:mapping-example}
\end{figure*}

\subsection{Construction of Mapping}
\label{sec:fullSecureMap}
We utilize private set operation protocols to build the mapping protocol. As a warm-up, we first present two constructions based on PSI and PID. Then, we present our fully secure mapping protocol.

\subsubsection{PSI-based mapping}
PSI protocols simply output the intersection to both parties, and we can directly use it to construct a level-0 mapping protocol. First, $\alice$ and $\bob$  run the PSI protocol to get the intersection. $\alice$ computes $\pi_a$ representing the sorting order on intersection elements such that $x_{\pi_a(i)} < x_{\pi_a(i + 1)}$ and $\forall x_j\in X\cap Y$, $j \in \pi_a$. $\bob$ computes $\pi_b$ similarly.  Two parties commonly set a length-$n_{xy}$ vector $E = (1, \dots, 1)$ as the intersection flag, where $n_{xy} = |X \cap Y|$. 

\begin{theorem}
    PSI-based mapping protocol satisfies level-0 security.
    \label{theorem:psi}
\end{theorem}

\begin{proof}
The PSI functionality\cite{kolesnikov2016efficient} outputs the set intersection, which means $E$ is revealed to both $\alice$ and $\bob$. It reveals nothing else due to the security guarantee of PSI. Thus the theorem holds.
\end{proof}

\subsubsection{PID-based mapping}
$\alice$ and $\bob$ first run the PID protocol. After receiving $(R^*, R(x_1), \dots, R(x_{n_x}))$, $\alice$ sorts $R^*$ in ascending order to get $P$, and computes a length-$|R^*|$ permutation $\pi_a$ satisfying $\forall i \in [|R^*|]$, if $\exists x_k \in X$ s.t. $R(x_k) = P_i$, then $\pi_a(i) = k$.
% with $\pi_a(i)\in[n_x]$, there is $R(x_{\pi_a(i)}) = P_i$.
Similarly, $\bob$ computes $\pi_b$. Then, two parties compute $\shareb{e_i} = \functionsym{eq}(x_{\pi_a(i)}, y_{\pi_b(i)})$ for $i\in [|P|]$ as the output.

\begin{theorem}
    PID-based mapping protocol satisfies level-1 security.
\end{theorem}

\begin{proof}
The functionality of PID \cite{buddhavarapu2020private} outputs $(R^*,M)$ to both parties as described in \ref{sec:map-related}. Since $|R^*|=|X \cup Y| $, the PID-based mapping naturally reveals $f(X,Y)$ , where $f$ outputs union size.  The identifiers in $R^*$ are generated randomly and $M$ only tells the mapping relation between self-owned input and the corresponding identifier in $R^*$,  and nothing else is leaked due to the security guarantee of PID. Thus the theorem holds.
\end{proof}

% \begin{itemize}
%     \item \textbf{PSI-based}: $\alice$ and $\bob$ first run the PSI protocol to directly get the intersection. $\alice$ computes $\pi_a$ representing the sorting on intersection elements such that $x_{\pi_a(i)} < x_{\pi_a(i + 1)}$ and $\forall x_j\in X\cap Y$, $j \in \pi_a$. Similarly, $\bob$ computes $\pi_b$ and two parties share length-$n_{xy}$ vector $E = (1, \dots, 1)$ as the output.
%     \item \textbf{PID-based}: $\alice$ and $\bob$ first run the private ID protocol. After receiving $(R^*, R(x_1), \dots, R(x_{n_x}))$, $\alice$ sorts $R^*$ in ascending order to get $P$, and computes a length-$|R^*|$ permutation $\pi_a$ satisfying $\forall i \in [|R^*|]$, if $\exists x_k \in X$ s.t. $R(x_k) = P_i$, then $\pi_a(i) = k$.
%     % with $\pi_a(i)\in[n_x]$, there is $R(x_{\pi_a(i)}) = P_i$.
%     Similarly, $\bob$ computes $\pi_b$. Then, two parties compute $\shareb{e_i} = \functionsym{eq}(x_{\pi_a(i)}, y_{\pi_b(i)})$ for $i\in [|P|]$ as the output.
% \end{itemize}

% 原版安全说明：The above two protocols leak information about $E$ to different degrees. 
% The PSI-based protocol outputs the set intersection, which means $E$ is revealed to both $\alice$  and $\bob$. Thus, it achieves level-0 security. For the PID-based protocol, the $E$ is secret to both parties with $|E| = |X\cap Y|$, which reveals the cardinality of the union, so it achieves level-1 security.
% 原版：During the execution of the PSI-based protocol, the revealed information is the set intersection, which can be simulated with $E$ and $\pi_a$ (or $\pi_b$) by $\alice$ (or $\bob$). Thus, it achieves level-0 security.
% The random encoding received by two parties during the PID-based protocol can essentially be simulated with $\pi_a$ or $\pi_b$, and $|E| = |X\bigcap Y|$ depends on the inputs $X$ and $Y$, so it achieves level-1 security.
% The PSI-based protocol only achieves level-2 security, and the PID-based one achieves level-1 security.

\subsubsection{Fully secure mapping}
The ideal functionality $\functionsym{map}$ of the level-2 secure mapping protocol for the case when $n_x \geq n_y$ is in Fig. \ref{function:mapping}. The case when $n_x < n_y$ can be simply covered by reversing the roles of two parties, such that $|E| = \mathsf{max}(n_x, n_y)$.
We describe our mapping protocol $\protocolsym{map2}$ in Fig.~\ref{protocol:mapping}, and an example of this procedure is shown in Fig.~\ref{fig:mapping-example}.

The protocol $\protocolsym{map2}$ can be divided into two phases. The first phase (steps 1-2) is to compute $E$ and $Z$, where $e_i$ indicates whether $x_{\pi_a(i)} \in X \cap Y$. $Z$ can be seen as a partial permutation, where for $i \in[n_x]$, if $e_i = 1$, $z_i$ is the index of $y_j$ who equals $x_{\pi_a(i)}$, and $z_i = 0$ otherwise. The purpose of the second phase (steps 3-8) is to replace the 0s in $Z$ with random values to make it become a length-$n_x$ permutation $\pi_b$, which is conducted by randomly mapping each index of a non-intersection element in $Y$ to a position $i$ where $e_i=0$.
To do this, the parties need to identify the non-intersection elements in $Y$, and it is done by the second invocation of circuit PSI in step 3.
If $n_x > n_y$, the parties pad zeros into $F'$.
To guarantee the randomness of $\pi_b$, the parties shuffle the index vector $O'$ in step 5. 
If we track an value $d\in[n_x]$ that $d > n_y$ or $y_d\notin X \bigcap Y$, $d$ will be shuffled to a random position $i$ in $L$ where $F_i = 0$ after step 5.
Then, through the correlation between $E$ and $F$, the parties map each value $l_i$ with $f'_i = 0$ into a position $j$ satisfying $e_j = 0$ to obtain $P^0$.
Since the numbers of 1 in $E$ and $F'$ are the same, the parties can sort $L$ in the order of $F'$ to obtain $P^1$, and then treat $P^1$ as the result of sorting $P^0$ in the order of $E$.
Specifically, the parties compute a shared permutation $\sigma_1$ representing a stable sorting of one-bit vector $F'$, and applying $\sigma_1^{-1}$ on $L$ will sort $L$ in order of $F'$.
As shown in Fig. \ref{fig:mapping-example}, $P^1 = (3^{\underline{0}}, 4^{\underline{0}}, 1^{\underline{1}}, 2^{\underline{1}})$.
% of put $d_y$ into a position in $P^1$ such that all values in $I_y^x$ are behind it.
% and the values of $D_y^x = \{1, 4\}$ are in the front of $I_y^x = \{2, 3\}$.
To reverse the sorting of $P^1$ in the order of $E$, the parties compute a shared permutation $\sigma_0$ representing a stable sorting of $E$, and apply $\sigma_0$ on $P^1$. Finally, $\pi_b$ is obtained with \smalltextsf{MUX} gates in step 8.

% It can be seen that after step 8, $\pi_b$ is a permutation satisfying the requirement defined in Fig. \ref{function:mapping}, and each value $\pi_b(d_x)$ with $\pi_a(d_x)\in D_x^y$ corresponds to a random index value in $D_y^x$.

% Note that $\share{E}$ can be easily obtained by invoking circuit PSI and oblivious generalized switch network. The main challenge lies in how to generate a required permutation $\pi_b$.
% As an entry point, we describe our oblivious mapping construction protocol for the case when two input sets $X, Y$ have equal size in Fig.\ref{protocol:mapping}.

% Firstly, $\bob$ set $O = (1, 2, \dots, n_y)$ as the payload values of circuit PSI. After the execution of step 2, $z'_i = j$ and $e_i = 1$ for $\pi_a(i) \in I_x^y$ with $x_{\pi_a(i)} = y_j$, or $z'_i = e_i = 0$ otherwise. 
% An example is shown in Fig. \ref{fig:mapping-example}.
% The purpose of the following steps is to ``complete'' shared vector $Z'$ into a permutation, and we clarify the correctness by tracking an index value $d_y\in D_y^x$.

% After step 5, $d_y$ will be shuffled to a random position $i$ in $L$, where $F'_i = 0$.
% A stable sort on one-bit vector $F'$ will sort the values in order of $(0, 1)$, so applying $\sigma_1^{-1}$ on $L$ will put $d_y$ into a position in $P^1$ such that all values in $I_y^x$ are behind it.
% As shown in Fig. \ref{fig:mapping-example}, the index values $D_y^x = \{4,1\}$ will be placed into the positions in front of $I_y^x = \{3,2\}$ with random order.

% $\sigma_0$ represents a stable sort of $E$, where $e_j = 1$ iff $\pi_a(j)\in I_x^y$ and $e_j = 0$ otherwise. 
% By applying $\sigma_0$ on $P^1$, the value $d_y$ will be placed into $P_{d_x}$ with $\pi_a(d_x)\in D_x^y$. 
% It can be seen that after step 8, $\pi_b$ is a permutation satisfying the requirement defined in Fig. \ref{function:mapping}, and each value $\pi_b(d_x)$ with $\pi_a(d_x)\in D_x^y$ corresponds to a random index value in $D_y^x$. This randomness is guaranteed through two random permutations $\rho_0, \rho_1$ inputted by $\alice, \bob$.

\begin{theorem}
    $\protocolsym{map2}$ satisfies level-2 security.
         \label{theorem:map}
\end{theorem}

\begin{proof} (sketch) For $\protocolsym{map2}$, the simulators for $\alice$ (or $\bob$) can be naturally constructed by invoking the simulators of the invoked functionalities and sampling random bits with the same length of the outputs of the invoked functionalities. Thus, we can easily prove $\protocolsym{map2}$ securely implement $\functionsym{map}$ in the ($\functionsym{cpsi}$, $\functionsym{osn}^s$, $\functionsym{shuffle}$, $\functionsym{perGen}$, $\functionsym{perm}^\mathsf{s}$, $\functionsym{invp}^\mathsf{s}$, $\functionsym{mux}$)-hybrid model. Thus the theorem holds.
\end{proof}

% 原版\subsubsection{Security analysis sketch}
% First, the correctness of $\protocolsym{map2}$ holds according to the above analysis.
% Second, the simulators for $\alice$ (or $\bob$) can be easily constructed by sampling random bits with the same length of the outputs of invoked ideal functionalities and invoking the simulators of ideal functionalities. Thus, we can easily prove Theorem \ref{theorem:map} and omit\PL{why omit} the detailed proof.
% % \noindent \textbf{Correctness.}

% \begin{theorem}
%     Fig. \ref{protocol:mapping} securely implement $\functionsym{map}$ when $n_x=n_y$ in the ($\functionsym{cpsi}, \functionsym{osn}^s, \functionsym{perGen}, \functionsym{perm}^\mathsf{s}, \functionsym{invp}^\mathsf{s}, \functionsym{mux}$)-hybrid model.
%     \label{theorem:map}
% \end{theorem}

\noindent\textbf{Complexity analysis}:
The underling protocols implementing $\functionsym{osn}^s, \functionsym{shuffle}, \functionsym{perm}^\mathsf{s}$ and $\functionsym{invp}^\mathsf{s}$ take $O(1)$ rounds and the communication cost of $O(n\log n)$ bits, where $n = max(n_x, n_y)$.
The protocols for $\functionsym{cpsi}, \functionsym{perGen}$ and $\functionsym{mux}$ takes the communication cost of $O(n)$ bits and $O(1)$ rounds.
Therefore, our protocol takes the communication cost of $O(n\log n)$ bits and $O(1)$ rounds.

